HHMR: Holistic Hand Mesh Recovery by Enhancing the Multimodal Controllability of Graph Diffusion Models

Recent years have witnessed a trend of the deep integration of the generation and reconstruction paradigms. In this paper, we extend the ability of controllable generative models for a more comprehensive hand mesh recovery task: direct hand mesh generation, inpainting, reconstruction, and fitting in a single framework, which we name as Holistic Hand Mesh Recovery (HHMR). Our key observation is that different kinds of hand mesh recovery tasks can be achieved by a single generative model with strong multimodal controllability, and in such a framework, realizing different tasks only requires giving different signals as conditions. To achieve this goal, we propose an all-in-one diffusion framework based on graph convolution and attention mechanisms for holistic hand mesh recovery. In order to achieve strong control generation capability while ensuring the decoupling of multimodal control signals, we map different modalities to a shared feature space and apply cross-scale random masking in both modality and feature levels. In this way, the correlation between different modalities can be fully exploited during the learning of hand priors. Furthermore, we propose Condition-aligned Gradient Guidance to enhance the alignment of the generated model with the control signals, which significantly improves the accuracy of the hand mesh reconstruction and fitting. Experiments show that our novel framework can realize multiple hand mesh recovery tasks simultaneously and outperform the existing methods in different tasks, which provides more possibilities for subsequent downstream applications including gesture recognition, pose generation, mesh editing, and so on.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Hand pose estimation and mesh reconstruction are hot topics in computer vision with various applications in fields such as VR, AR, and biorobotics. However, in practical scenarios, these problems are often either ill-posed, such as reconstructing 3D hand mesh from a 2D RGB image, or with highly uncertainty, such as estimating hand poses from images with occlusions and motion blur. To address these issues, acquiring an appropriate prior distribution of human hand is important, which can help distinguish unfeasible postures and generate multitude plausible results with noisy observation. 

% Several hand prior has been explored in pervious works. Adrian Spurr \etal  proposed a set of biomechanically inspired constraints as hand skeleton's prior. However, skeleton based prior lacks hand shape information which is very important in contact situation. Based on parametric model, MANO utilzed principal component analysis (PCA) to formulate both hand pose and shape prior. Binghui Zuo \etal trained an VAE to build prior of two interacting human hands. However, the parameter space is highly nonlinear and not directly related to the 3D context (such as 3D joints), which means additional optimization process is required when applied to downstream tasks.

% In this work, we propose DiffHand, a new approach to learn 3D human hand prior for general purposes. Our method is a diffusion based method, which gradually denoise randomly point cloud and yield hand mesh. With differnt gaussian noise introduced in the denoising steps, our method can generate different reasonable hand meshes. To further enhance the functionality our model, we trainned our diffusion model with different condition to match different downstream tasks. For example, our diffusion model can take latent feature encoded from image as condition to generate hand meshed that align to the image. In this situation, our method works as a hand reconstruction network. Also, our model can take 2D joints as condition and work as a neural fitting network. We also applied random masking strategy on conditions, which masks our model can generate varied hand meshes with incomplete observation, such as occlusion image or incomplete 2D joints.

% To get better alignment with conditions, we adopt the method from ControlNet and classify guidance diffusion to improve generate result. (TODO)

% We summarize our contributions as follows:

% • We introduce DiffHand, a novel diffusion-based generative network to model 3D human hand prior general tasks.

% • We design different strategy to improve the consistence with condition.

% • We extend our single hand prior model to temporal prior model and interacting two hands prior model.

% hand-centered problem have long been a focal point in the field of visual perception, including hand gesture detection, pose estimation, motion tracking, and more. With the advent of differentiable parameterized hand templates, researchers have also turned their attention to single-image hand reconstruction. 


Hand pose estimation and mesh reconstruction are hot topics in computer vision with various applications in fields such as VR, AR, and biorobotics. Existing methods often employ regression approaches. Typically, these methods first use an encoder network to extract various information from input (monocular image, 2D skeletons \etc.), then either regress 3D hand poses \cite{spurr2020biomechanical}, predict the pose and shape parameters \cite{chen2021model,zhou2020monocular,boukhayma20193d,Zhang_2019_ICCV} of a parametric hand model \cite{MANO:SIGGRAPHASIA:2017} or directly regress the vertex coordinates of a 3D hand mesh \cite{Ge_2019_CVPR,chen2021cameraspace,tang2021towards,chen2022mobrecon,kulon2020weakly,lin2021mesh,lin2021metro} by a regression decoder. However, due to the complexity of hand poses, the input is often constrained, such as occluded images or incomplete 2D skeletons. Which increases the complexity and uncertainty of hand pose estimation and mesh reconstruction. Considering the biomechanical constraints, plausible hand poses lie on a low-dimensional manifold distribution within full poses space\cite{tiwari2022posendf}. Acquiring such a prior distribution not only facilitates the pose estimation and reconstruction tasks but also enables the sampling of diverse postures.

Hence, various types of prior models for human hands have been proposed. In an explicit manner, Spurr \etal \cite{spurr2020biomechanical} constrain the bone length and the adjacent bone angles to lie in a plausible range, while Yang \etal \cite{Yang_2021_ICCV_CPF} directly restrict the degrees of freedom (DoF) for each hand joint and constrain the rotation angle of each DoF. Romero \etal \cite{MANO:SIGGRAPHASIA:2017} employed principal component analysis (PCA) on the pose and shape parameters of the hand dataset to establish priors. However, these explicit priors either rely on manually defined constraints or are based on simple linear analysis, thus unable to represent complex postures or generate diverse hand meshes \yt{(Important Task?)}. 
Others have explored learning-based implicit generative models as priors for the human hand. Some researchers \cite{zuo2023twohandvae,li2021task} have utilized the Variational Autoencoder (VAE) to map the parameters to a Gaussian space. By leveraging these priors, it becomes possible to generate hand models through sampling in feasible distributions. Some researchers have also explored using VAE to encode the image domain and hand pose domain, then utilize CrossVAE or Generative Adversarial Network (GAN) to align these two domains, enabling the generation of hand from input image (\cite{wan2017crossing,spurr2018cross,yang2019aligning,yang2019disentangling}). 
These implicit prior models are mostly built on the parameter space of hand templates or hand 3D skeletons. When introducing geometric constraints, additional inversion processes are required, which is unstable and time-consuming. 

We believe that the two tasks mentioned above - hand reconstruction and generative hand prior modeling - can be viewed as one unified task. The reconstruction task can be seen as generation task under specific conditions. For instance, given an occlusion hand image as input, we expect the generation model could yield multiple hands, which are aligned with hand visible image part and various on the occluded image part. In this case, we take the image hand reconstruction task as image conditional hand generation task. Also, given incomplete 2D/3D hand skeleton as input, the generation model should generate hand meshes that match the input skeleton. In this case, we take the hand pose estimation task as skeleton conditional hand generation task. In the human body reconstruction and pose estimation tasks, some researchers have also considered this unification to generation task (\cite{wan2017crossing,spurr2018cross,yang2019aligning,yang2019disentangling}). However, these approaches either do not consider the alignment with the given conditions or only provide skeletal output. Furthermore, there are currently no similar methods available specifically for hand reconstruction. 

Thus, we propose a new approach to generate hand mesh from various conditions. Our method is a diffusion-based method that directly processes 3D hand meshes, which gradually denoise point clouds to yield plausible hand meshes. Our generation model is conditional either on RGB image, 2D/3D skeleton, or the combination of them according to specific tasks, which allows our model to apply to various downstream tasks. 
We also applied a random masking strategy on conditions, which masks our model can generate varied hand meshes with incomplete observation, such as occlusion images or incomplete 2D joints, or work as an unconditional generate model. 
Finally, we adopted the classifier guidance diffusion method to further increase the alignment with the conditions. Further experiments demonstrate the effectiveness of our approach on various generation, completion, reconstruction, and fitting tasks. 

We summarize our contributions as follows:

• We introduce a novel diffusion-based generative network that directly process on hand meshes.

• We design a task-specific conditional input training method, allowing our approach with various downstream applications.

• We design classifier guidance based strategy to further improve the alignment with condition.

% • We introduce a novel diffusion-based generative network to model 3D human hand prior with various conditions.

% • We introduce a diffusion-based generative method for hand reconstruction and pose estimation.

% • We design classifier guidance based strategy to further improve the alignment with condition.

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

% [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

